HyperFair: A Soft Approach to Integrating Fairness Criteria

Recommender systems are being employed across an increasingly diverse set of domains that can potentially make a significant social and individual impact. For this reason, considering fairness is a critical step in the design and evaluation of such systems. In this paper, we introduce HyperFair, a general framework for enforcing soft fairness constraints in a hybrid recommender system. HyperFair models integrate variations of fairness metrics as a regularization of a joint inference objective function. We implement our approach using probabilistic soft logic and show that it is particularly well-suited for this task as it is expressive and structural constraints can be added to the system in a concise and interpretable manner. We propose two ways to employ the methods we introduce: first as an extension of a probabilistic soft logic recommender system template; second as a fair retrofitting technique that can be used to improve the fairness of predictions from a black-box model. We empirically validate our approach by implementing multiple HyperFair hybrid recommenders and compare them to a state-of-the-art fair recommender. We also run experiments showing the effectiveness of our methods for the task of retrofitting a black-box model and the trade-off between the amount of fairness enforced and the prediction performance.

==> sections/related_work.tex <==
\section{Related Works}
\label{sec:Related Works}

% One paragraph to review related works. Citing lots of FAccTRec people.
Generally methods for addressing unfairness can fall into three stages of a pipeline: pre-process, in-process, and post-process \cite{mehrabi2019survey}.
% pre process fairness
Pre-processing techniques transform the data so that discrimination characteristics are removed prior to model training \cite{lahoti2019ifair, NIPS2017_6988}.
Our work does not fit into this category of techniques but instead can be viewed as either an in-processing or post-processing method.
% post processing fairness
Post-processing techniques treat the learned model as a black box and modify the output to remove discrimination \cite{FairnessExposureInRankings:Singh,  equalityOfOpportunity:Hardt, LinkedInReRanking:Geyik, MatchmakingFairness:Paraschakis}.
This class of approach is a simple way to integrate fairness constraints into an existing pipeline, which is a common practical requirement for industry applications \cite{AdressingAlgorithmicBias:Gathright, LinkedInReRanking:Geyik}
% in process fairness
In-processing techniques attempt to remove discrimination during the model training process, either by incorporating changes into the objective function or by imposing a constraint.
%Adversarial learning
Recent work has shown the effectiveness of both adversarial learning
\cite{AdversariallyLearningFairRepresentations:Beutel, Louizos:CoRR2016, Madras:CoRR2018} 
% Fairness via regularization
and regularization \cite{FairnessAwareRegularizer, DBLP:journals/corr/YaoH17, PairwiseFairness} 
as in-processing methods for addressing fairness.
Our work specifically builds upon the line of research that addresses fairness via regularization.
